Assurance Monitoring of Cyber-Physical Systems with Machine Learning Components

Machine learning components such as deep neural networks are used extensively in Cyber-Physical Systems (CPS). However, they may introduce new types of hazards that can have disastrous consequences and need to be addressed for engineering trustworthy systems. Although deep neural networks offer advanced capabilities, they must be complemented by engineering methods and practices that allow effective integration in CPS. In this paper, we investigate how to use the conformal prediction framework for assurance monitoring of CPS with machine learning components. In order to handle high-dimensional inputs in real-time, we compute nonconformity scores using embedding representations of the learned models. By leveraging conformal prediction, the approach provides well-calibrated confidence and can allow monitoring that ensures a bounded small error rate while limiting the number of inputs for which an accurate prediction cannot be made. Empirical evaluation results using the German Traffic Sign Recognition Benchmark and a robot navigation dataset demonstrate that the error rates are well-calibrated while the number of alarms is small. The method is computationally efficient, and therefore, the approach is promising for assurance monitoring of CPS.

==> tables/epislon_selection_scitos.tex <==
\begin{table}[H]
\fontsize{11}{13}\selectfont
\centering
    \begin{tabularx}{\linewidth}{| X | c | c | c |}
        \hline
        \multicolumn{4}{|c|}{$\epsilon=0.01$} \\
        \hline
        NC Functions     & Errors \% & Multiples \% & Empty \% \\ \hhline{|=|=|=|=|}
        Multiple Neighbors & 0.7\% & 62.6\% & 0 \\ \hline
        1 Neighbor         & 1.8\% & 43.6\% & 0 \\ \hline
        Nearest Centroid & 0.9\% & 94\% & 0  \\ \hline
        Margin & 0.7\% & 58.6\% & 0\\ \hline
        Brier Score & 0.7\% & 58.8\% & 0\\ \hline
        Margin Scaled & 0.9\% & 52.2\% & 0\%\\ \hline
        Brier Score Scaled & 0.9\% & 52.2\% & 0\\ \hline
    \end{tabularx}
    \caption{$\epsilon$ selection for the SCITOS-G5 dataset}
    \label{tab:epsilon_selection_scitos}
\end{table}

==> tables/epsilon_calculation_everything_old.tex <==
\begin{table*}[ht]
\fontsize{11}{13}\selectfont
	\centering
	{\renewcommand{\arraystretch}{1.2}
		\begin{tabular}{c||c|c|c|c|}
			\cline{2-5}
			  & \multicolumn{4}{|c|}{Calculate $\epsilon$}\\\hline
			Dataset & NC Functions & $\epsilon$ & Errors & Multiples \\ \hline\hline
			\multirow{7}{*}{GTSRB} & Multiple Neighbors & 0.021 & 2.3\% & 0  \\\cline{2-5}
			& 1 Neighbor & 0.016 & 2.3\% & 0 \\\cline{2-5}
			& Nearest Centroid & 0.026 & 2.8\% & 0 \\\cline{2-5}
			& Margin & 0.034 & 3.4\% & 0\\ \cline{2-5}
            & Brier Score & 0.035 & 3.6\% & 0\\ \cline{2-5}
            & Margin Scaled & 0.034 & 3.4\% & 0\\ \cline{2-5}
            & Brier Score Scaled & 0.035\% & 3.6\% & 0\\ \hline\hline
			\multirow{7}{*}{SCITOS-G5} & Multiple Neighbors & 0.088 & 8.7\% & 11.3\% \\\cline{2-5}
			& 1 Neighbor & 0.092 & 10.4\% & 0 \\\cline{2-5}
			& Nearest Centroid & 0.099 & 8.8\% & 75.2\% \\\cline{2-5}
			& Margin & 0.1 & 10.6\% & 4.7\%\\ \cline{2-5}
            & Brier Score & 0.1 & 10.6\% & 4.8\%\\ \cline{2-5}
            & Margin Scaled & 0.1 & 10.6\% & 4.4\%\\ \cline{2-5}
            & Brier Score Scaled & 0.1 & 10.8\% & 4.6\% \\\hline
		\end{tabular}
		\vspace*{0.1in}
	}
	\caption{\textbf{Adversarial example classification accuracy for the DNN and DkNN}: attack parameters are chosen according to prior work. All input features were clipped to
	remain in their range. Note that most wrong predictions made by the DkNN are assigned low credibility (see Figure~\ref{fig:dknn-relia-diag-adv-ex} and the Appendix).}
	\label{tbl:adv-ex-detection}
\end{table*}

==> tables/epsilon_calculation_gtsrb.tex <==
\begin{table}[H]
\centering
    \begin{tabularx}{\linewidth}{| X | c | c | c |}
        \hline
        NC Functions     & $\epsilon$ & Errors & Multiples \\ \hhline{|=|=|=|=|}
        %\hline\hline
        Multiple Neighbors & 0.021 & 2.3\% & 0 \\ \hline
        1 Neighbor         & 0.016 & 2.3\% & 0 \\ \hline
        Nearest Centroid & 0.026 & 2.8\% & 0  \\ \hline
        Margin & 0.034 & 3.4\% & 0\\ \hline
        Brier Score & 0.035 & 3.6\% & 0\\ \hline
        Margin Scaled & 0.034 & 3.4\% & 0\\ \hline
        Brier Score Scaled & 0.035\% & 3.6\% & 0\\ \hline
    \end{tabularx}
    \caption{$\epsilon$ estimation for the GTSRB dataset}
    \label{tab:epsilon_estimation_gtsrb}
\end{table}

==> tables/epsilon_calculation_scitos.tex <==
\begin{table}[H]
\centering
    \begin{tabularx}{\linewidth}{| X | c | c | c |}
        \hline
        NC Functions     & $\epsilon$ & Errors & Multiples \\ \hhline{|=|=|=|=|}
        %\hline\hline
        Multiple Neighbors & 0.088 & 8.7\% & 11.3\% \\ \hline
        1 Neighbor         & 0.092 & 10.4\% & 0 \\ \hline
        Nearest Centroid & 0.099 & 8.8\% & 75.2\%  \\ \hline
        Margin & 0.1 & 10.6\% & 4.7\%\\ \hline
        Brier Score & 0.1 & 10.6\% & 4.8\%\\ \hline
        Margin Scaled & 0.1 & 10.6\% & 4.4\%\\ \hline
        Brier Score Scaled & 0.1 & 10.8\% & 4.6\%\\ \hline
    \end{tabularx}
    \caption{$\epsilon$ estimation for the SCITOS-G5 dataset}
    \label{tab:epsilon_estimation_scitos}
\end{table}

==> tables/epsilon_selection_gtsrb.tex <==
\begin{table}[H]
\fontsize{11}{13}\selectfont
\centering
    \begin{tabularx}{\linewidth}{| X | c | c | c |}
        \hline
        \multicolumn{4}{|c|}{$\epsilon=0.01$} \\
        \hline
        NC Functions     & Errors \% & Multiples \% & Empty \% \\ \hhline{|=|=|=|=|}
        Multiple Neighbors & 1.1\% & 3.5\% & 0 \\ \hline
        1 Neighbor         & 1.3\% & 2.1\% & 0 \\ \hline
        Nearest Centroid & 1.2\% & 4.8\% & 0  \\ \hline
        Margin & 0.9\% & 7.1\% & 0\\ \hline
        Brier Score & 0.9\% & 7.1\% & 0\\ \hline
        Margin Scaled & 0.7\% & 8.8\% & 0\\ \hline
        Brier Score Scaled & 0.7\% & 8.8\% & 0\\ \hline
    \end{tabularx}
    \caption{$\epsilon$ selection for the GTSRB dataset}
    \label{tab:epsilon_selection_gtsrb}
\end{table}
